A Singular Value Perspective on Model Robustness

Convolutional Neural Networks (CNNs) have made significant progress on several computer vision benchmarks, but are fraught with numerous non-human biases such as vulnerability to adversarial samples. Their lack of explainability makes identification and rectification of these biases difficult, and understanding their generalization behavior remains an open problem. In this work we explore the relationship between the generalization behavior of CNNs and the Singular Value Decomposition (SVD) of images. We show that naturally trained and adversarially robust CNNs exploit highly different features for the same dataset. We demonstrate that these features can be disentangled by SVD for ImageNet and CIFAR-10 trained networks. Finally, we propose Rank Integrated Gradients (RIG), the first rank-based feature attribution method to understand the dependence of CNNs on image rank.

==> cvpr.tex <==
% % This version of CVPR template is provided by Ming-Ming Cheng.
% % Please leave an issue if you found a bug:
% % https://github.com/MCG-NKU/CVPR_Template.

% % \documentclass[review]{cvpr}
% \documentclass[final]{cvpr}

% \usepackage{times}
% \usepackage{epsfig}
% % \usepackage{ulem}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{algorithmic}
% \usepackage{caption}
% \usepackage{subcaption}
% \captionsetup{compatibility=false}
% \usepackage[T1]{fontenc}
% \pdfoutput=1

% % Include other packages here, before hyperref.

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}


% \def\cvprPaperID{10725} % *** Enter the CVPR Paper ID here
% \def\confYear{CVPR 2021}
% %\setcounter{page}{4321} % For final version only


% \begin{document}

% %%%%%%%%% TITLE
% \title{A Singular Value Perspective on Model Robustness}

% \author{Malhar Jere\\
% UC San Diego\\
% {\tt\small mjjere@ucsd.edu}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Maghav Kumar\\
% UIUC\\
% {\tt\small mkumar10@illinois.edu}

% \and
% Farinaz Koushanfar\\
% UC San Diego\\
% {\tt\small fkoushanfar@ucsd.edu}}
% \maketitle


% %%%%%%%%% ABSTRACT
% \begin{abstract}
% %   Convolutional Neural Networks (CNNs) have achieved impressive achievements on several computer vision tasks, but are fraught with numerous non-human biases such as vulnerability to adversarial samples. Their lack of explainability makes identification and rectification of these biases difficult, and understanding the generalization behavior of CNNs remains an open problem. In this work we explore the relationship between the generalization behavior of CNNs and the Singular Value Decomposition (SVD) of images. 
% %   We show that naturally trained and adversarially robust CNNs for the ImageNet and CIFAR-10 datasets exploit highly different features for the same dataset and show that these features can be disentangled by low-rank approximation. Finally, we propose \textbf{R}ank \textbf{I}ntegrated \textbf{G}radients \textbf{(RIG)}, the first rank-based feature attribution method to understand the dependence of CNNs on image rank.
  
%   Convolutional Neural Networks (CNNs) have made significant progress on several computer vision benchmarks, but are fraught with numerous non-human biases such as vulnerability to adversarial samples. Their lack of explainability makes identification and rectification of these biases difficult, and understanding their generalization behavior remains an open problem. In this work we explore the relationship between the generalization behavior of CNNs and the Singular Value Decomposition (SVD) of images. We show that naturally trained and adversarially robust CNNs exploit highly different features for the same dataset. We demonstrate that these features can be disentangled by SVD for ImageNet and CIFAR-10 trained networks. Finally, we propose \textbf{R}ank \textbf{I}ntegrated \textbf{G}radients \textbf{(RIG)}, the first rank-based feature attribution method to understand the dependence of CNNs on image rank. 
% %   We show that naturally trained neural networks exploit features that are useful for predictions yet incomprehensible to humans. 
% %   We further demonstrate that naturally trained and adversarially robust neural networks exploit highly different features for the same dataset. We show that these features can be disentangled by low-rank approximation, and establish the existence of such features in the CIFAR-10 and ImageNet datasets.
% \end{abstract}

% \vspace{-20pt}

% %%%%%%%%% BODY TEXT
% \input{latex/1_introduction}

% \input{latex/2_background}

% \input{latex/3_methodology}

% \input{latex/4_rank_truncation}

% \input{latex/5_transferability}

% \input{latex/6_discussion}

% \input{latex/7_conclusion}

% \input{latex/8_acknowledgements}
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{cvpr}
% }

% \input{latex/9_appendix}



% \end{document}

% % \documentclass[review]{cvpr}
% \documentclass[final]{cvpr}

% \usepackage{times}
% \usepackage{epsfig}
% % \usepackage{ulem}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{algorithmic}
% \usepackage{caption}
% \usepackage{subcaption}
% \captionsetup{compatibility=false}
% \usepackage[T1]{fontenc}
% \pdfoutput=1

% % Include other packages here, before hyperref.

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}


% \def\cvprPaperID{10725} % *** Enter the CVPR Paper ID here
% \def\confYear{CVPR 2021}
% %\setcounter{page}{4321} % For final version only


% \begin{document}

% %%%%%%%%% TITLE
% \title{A Singular Value Perspective on Model Robustness}

% \author{Malhar Jere\\
% UC San Diego\\
% {\tt\small mjjere@ucsd.edu}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Maghav Kumar\\
% UIUC\\
% {\tt\small mkumar10@illinois.edu}

% \and
% Farinaz Koushanfar\\
% UC San Diego\\
% {\tt\small fkoushanfar@ucsd.edu}}
% \maketitle


% %%%%%%%%% ABSTRACT
% \begin{abstract}
% %   Convolutional Neural Networks (CNNs) have achieved impressive achievements on several computer vision tasks, but are fraught with numerous non-human biases such as vulnerability to adversarial samples. Their lack of explainability makes identification and rectification of these biases difficult, and understanding the generalization behavior of CNNs remains an open problem. In this work we explore the relationship between the generalization behavior of CNNs and the Singular Value Decomposition (SVD) of images. 
% %   We show that naturally trained and adversarially robust CNNs for the ImageNet and CIFAR-10 datasets exploit highly different features for the same dataset and show that these features can be disentangled by low-rank approximation. Finally, we propose \textbf{R}ank \textbf{I}ntegrated \textbf{G}radients \textbf{(RIG)}, the first rank-based feature attribution method to understand the dependence of CNNs on image rank.
  
%   Convolutional Neural Networks (CNNs) have made significant progress on several computer vision benchmarks, but are fraught with numerous non-human biases such as vulnerability to adversarial samples. Their lack of explainability makes identification and rectification of these biases difficult, and understanding their generalization behavior remains an open problem. In this work we explore the relationship between the generalization behavior of CNNs and the Singular Value Decomposition (SVD) of images. We show that naturally trained and adversarially robust CNNs exploit highly different features for the same dataset. We demonstrate that these features can be disentangled by SVD for ImageNet and CIFAR-10 trained networks. Finally, we propose \textbf{R}ank \textbf{I}ntegrated \textbf{G}radients \textbf{(RIG)}, the first rank-based feature attribution method to understand the dependence of CNNs on image rank. 
% %   We show that naturally trained neural networks exploit features that are useful for predictions yet incomprehensible to humans. 
% %   We further demonstrate that naturally trained and adversarially robust neural networks exploit highly different features for the same dataset. We show that these features can be disentangled by low-rank approximation, and establish the existence of such features in the CIFAR-10 and ImageNet datasets.
% \end{abstract}

% \vspace{-20pt}

% %%%%%%%%% BODY TEXT
% \input{latex/1_introduction}

% \input{latex/2_background}

% \input{latex/3_methodology}

% \input{latex/4_rank_truncation}

% \input{latex/5_transferability}

% \input{latex/6_discussion}

% \input{latex/7_conclusion}

% \input{latex/8_acknowledgements}
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{cvpr}
% }

% \input{latex/9_appendix}



% \end{document}

